DALR: Dual-level Alignment Learning for Multimodal Sentence Representation Learning

Previous multimodal sentence representation learning methods have achieved impressive performance. However, most approaches focus on aligning images and text at a coarse level, facing two critical challenges:cross-modal misalignment bias and intra-modal semantic divergence, which significantly degrade sentence representation quality. To address these challenges, we propose DALR (Dual-level Alignment Learning for Multimodal Sentence Representation). For cross-modal alignment, we propose a consistency learning module that softens negative samples and utilizes semantic similarity from an auxiliary task to achieve fine-grained cross-modal alignment. Additionally, we contend that sentence relationships go beyond binary positive-negative labels, exhibiting a more intricate ranking structure. To better capture these relationships and enhance representation quality, we integrate ranking distillation with global intra-modal alignment learning. Comprehensive experiments on semantic textual similarity (STS) and transfer (TR) tasks validate the effectiveness of our approach, consistently demonstrating its superiority over state-of-the-art baselines.

==> tables/cross_modal_retrieval.tex <==
\begin{table}[h]
 
 \begin{center}
 \scalebox{0.85}{
  \begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{\text{image } $\rightarrow$ \text{text}}} &
    \multicolumn{2}{c}{\textbf{\text{text } $\rightarrow$ \text{image}}}\\
    \cmidrule{2-5}
     & R@1 & R@5 & R@1 & R@5 \\
    \midrule
    \midrule
    MCSE\textsubscript{\textit{wiki+flickr}} & 16.7&	43.5&	22.5 &	50.4  \\
    KDMCSE\textsubscript{\textit{wiki+flickr}} & 17.9&	45.0&	24.1 &	52.8  \\
    \quad \quad w/ CML & 19.1 & 46.4 & 25.6 & 54.0  \\
    DALR\textsubscript{\textit{wiki+flickr}} & 19.5&	47.6&	26.7 &	55.9  \\
    \midrule
    MCSE\textsubscript{\textit{wiki+coco}} & 8.8&	26.6&	10.9&	31.2  \\
    KDMCSE\textsubscript{\textit{wiki+coco}} & 9.4& 27.9&	12.2&	32.7  \\
    \quad \quad w/ CML & 9.7 & 28.6 & 13.3 & 33.9  \\
     DALR\textsubscript{\textit{wiki+coco}} & 10.2&	29.0&	13.9&	34.3  \\
  
  \bottomrule
  \end{tabular}} \\
  \caption{Multimodal retrieval results on Flickr30k test set based on BERT$_\text{base}$. }
 
  \label{tab:cross_modal_retrieval}
  \end{center}
\end{table}

==> tables/sentence_retrieval.tex <==

\begin{table*}[t]
\caption{Retrieved examples from Flickr30k test set.}
 \begin{center}
 \scalebox{0.95}{
  \begin{tabular}{ll}
  \toprule
  \textbf{Model} & \textbf{Result} \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 1}: A young girl is washing her teddy bear in the kitchen sink. } \\
  \midrule
  SimCSE: & A middle-aged woman is vacuuming her kitchen floor with a canister vac.   \\
  MCSE: & A young girl, blond and wearing a polka-dot shirt, washes a stuffed animal in a vanity sink. \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 2}: Three chefs , wearing white hats and black aprons , are preparing food in a crowded kitchen.} \\
  \midrule
  SimCSE: &  Numerous workers with blue shirts and white aprons are preparing fish for sale.  \\
  MCSE: & Three men are preparing food in a kitchen setting. \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 3}: A couple kisses in a shady walkway. } \\
  \midrule
  SimCSE: &   A couple strolls down a path near benches and water. \\
  MCSE: & Couple kissing outside on street. \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 4}: A man is standing on the streets taking photographs. } \\
  \midrule
  SimCSE: &   People run a marathon on a city street with a crowd watching.  \\
  MCSE: &   A guy wearing a white shirt is taking a picture. \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 5}: Two boys are playing in pool filled with sparkling blue water. } \\
  \midrule
  SimCSE: &   A little girl is swimming under the crystal blue water.  \\
  MCSE: & Two children are swimming in a pool. \\
  \midrule
  \multicolumn{2}{l}{\textbf{Query 6}: An old man sitting on a bench staring at the ocean.} \\
  SimCSE: &  A man sitting on a bench by the ocean.  \\
  MCSE: & An old man sits on a bench overlooking the water. \\
  \bottomrule
  \end{tabular}}
  
  \label{tb:sentence_retrieval}
  \end{center}
\end{table*}

